Meta Learning-based MIMO Detectors: Design, Simulation, and Experimental Test

Deep neural networks (NNs) have exhibited considerable potential for efficiently balancing the performance and complexity of multiple-input and multiple-output (MIMO) detectors. We propose a receiver framework that enables efficient online training by leveraging the following simple observation: although NN parameters should adapt to channels, not all of them are channel-sensitive. In particular, we use a deep unfolded NN structure that represents iterative algorithms in signal detection and channel decoding modules as multi layer deep feed forward networks. An expectation propagation (EP) module, called EPNet, is established for signal detection by unfolding the EP algorithm and rendering the damping factors trainable. An unfolded turbo decoding module, called TurboNet, is used for channel decoding. This component decodes the turbo code, where trainable NN units are integrated into the traditional max-log-maximum a posteriori decoding procedure. We demonstrate that TurboNet is robust for channels and requires only one off-line training. Therefore, only a few damping factors in EPNet must be re-optimized online. An online training mechanism based on meta learning is then developed. Here, the optimizer, which is implemented by long short-term memory NNs, is trained to update damping factors efficiently by using a small training set such that they can quickly adapt to new environments. Simulation results indicate that the proposed receiver significantly outperforms traditional receivers and that the online learning mechanism can quickly adapt to new environments. Furthermore, an over-the-air platform is presented to demonstrate the significant robustness of the proposed receiver in practical deployment.

==> macro.TeX <==


    %\newcommand{\tr}{\mbox{trace}}
    \def\bm#1{\boldsymbol{#1}}
    \def\ang#1{\mbox{$\langle #1 \rangle$}}
    \def\aang#1{\mbox{$\langle\!\langle #1 \rangle\!\rangle$}}

    \def\mnorm#1{\mbox{$\left|\!\left|\!\left|\, #1 \,\right|\!\right|\!\right|$}}



    \def\Complex{{\rm\rule[.23ex]{.03em}{1.1ex}\kern-.3em{C}}}
    \def\bms#1{\mbox{\boldmath $\scriptstyle #1$}}
    \def\eqover#1{\mbox{$\buildrel #1 \over =$}}
    \def\leqover#1{\mbox{$\buildrel #1 \over \leq$}}
    \def\Imag#1{\mbox{${\Im}\left\{ #1 \right\}$}}
    \def\dist{\mbox{${\sf dist}(z, {\mathbb R}^+)$}}
    \def\largeN{\mbox{${\cal N}$}}

    \newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}}
    \newcommand{\bea}{\begin{eqnarray}} \newcommand{\eea}{\end{eqnarray}}
    \newcommand{\benum}{\begin{enumerate}} \newcommand{\eenum}{\end{enumerate}}
    \def\proof{\noindent\hspace{2em}{\itshape Proof: }}
    \def\aproof{\noindent\hspace{2em}{\itshape Alternative Proof: }}
    \def\endproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}
    \def\endaproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}

  %\newtheorem{theorem}{Theorem}
  %\newtheorem{conjecture}{Conjecture}
  %\newtheorem{definition}{Definition}
  %\newtheorem{example}{Example}
  %\newtheorem{lemma}{Lemma}
  %\newtheorem{proposition}{Proposition}
  %\newtheorem{claim}{Claim}

  \def \veclen {0.8}
  \def \uppos{1.2}
  \def \lowpos{-1.5}
  \def \recwid{0.6}
  \def \rechig{0.4}
  \def \crad{0.25}

  \def \Fwid{0.8}

  \newcommand{\tbox}[1]{%

     \bsegment
      \realmult {\rechig}{0.5} \ta
      \realmult {\recwid}{0.5} \tb
       \lvec (0 \ta)    \lvec ({\recwid} \ta)
       \lvec ({\recwid} -\ta) \lvec (0 -\ta)\lvec (0 0)
       \textref h:C v:C \htext ({\tb} 0){#1}
       \savepos ({\recwid} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}

  \newcommand{\tcir}[1]{%
     \bsegment
     \realmult {\crad}{2} \ta
       \move({\crad} 0)
       \lcir r:{\crad}
       \textref h:C v:C \htext ({\crad} 0) {#1}
       \savepos ({\ta} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}


  \newcommand{\tupnoisec}[1]{%
     \bsegment
     \realadd{\crad}{0.35}\arrowlen
     \realadd{\arrowlen}{0.08}\txtpos
     \rmove({-\crad} \arrowlen) \avec({-\crad} \crad)
     \textref h:C v:C \htext ({-\crad} \txtpos){#1}
     \esegment}

    %%%%%% DEFINITION %%%%%%%%%%%%%%
    \newcommand{\qa}{{\bf a}}
    \newcommand{\qb}{{\bf b}}
    \newcommand{\qc}{{\bf c}}
    \newcommand{\qd}{{\bf d}}
    \newcommand{\qe}{{\bf e}}
    \newcommand{\qf}{{\bf f}}
    \newcommand{\qg}{{\bf g}}
    \newcommand{\qh}{{\bf h}}
    \newcommand{\qi}{{\bf i}}
    \newcommand{\qj}{{\bf j}}
    \newcommand{\qk}{{\bf k}}
    \newcommand{\ql}{{\bf l}}
    \newcommand{\qm}{{\bf m}}
    \newcommand{\qn}{{\bf n}}
    \newcommand{\qo}{{\bf o}}
    \newcommand{\qp}{{\bf p}}
    \newcommand{\qq}{{\bf q}}
    \newcommand{\qr}{{\bf r}}
    \newcommand{\qs}{{\bf s}}
    \newcommand{\qt}{{\bf t}}
    \newcommand{\qu}{{\bf u}}
    \newcommand{\qv}{{\bf v}}
    \newcommand{\qw}{{\bf w}}
    \newcommand{\qx}{{\bf x}}
    \newcommand{\qy}{{\bf y}}
    \newcommand{\qz}{{\bf z}}

    \newcommand{\qA}{{\bf A}}
    \newcommand{\qB}{{\bf B}}
    \newcommand{\qC}{{\bf C}}
    \newcommand{\qD}{{\bf D}}
    \newcommand{\qE}{{\bf E}}
    \newcommand{\qF}{{\bf F}}
    \newcommand{\qG}{{\bf G}}
    \newcommand{\qH}{{\bf H}}
    \newcommand{\qI}{{\bf I}}
    \newcommand{\qJ}{{\bf J}}
    \newcommand{\qK}{{\bf K}}
    \newcommand{\qL}{{\bf L}}
    \newcommand{\qM}{{\bf M}}
    \newcommand{\qN}{{\bf N}}
    \newcommand{\qO}{{\bf O}}
    \newcommand{\qP}{{\bf P}}
    \newcommand{\qQ}{{\bf Q}}
    \newcommand{\qR}{{\bf R}}
    \newcommand{\qS}{{\bf S}}
    \newcommand{\qT}{{\bf T}}
    \newcommand{\qU}{{\bf U}}
    \newcommand{\qV}{{\bf V}}
    \newcommand{\qW}{{\bf W}}
    \newcommand{\qX}{{\bf X}}
    \newcommand{\qY}{{\bf Y}}
    \newcommand{\qZ}{{\bf Z}}
    \newcommand{\qzero}{{\bf 0}}
    \newcommand{\qone}{{\bf 1}}
    \newcommand{\qdh}{\triangle\qh}
    \newcommand{\qhh}{\hat\qh}
    \newcommand{\qdH}{\triangle\qH}
    \newcommand{\qhH}{\hat\qH}
    \newcommand{\qdF}{\triangle\qF}
    \newcommand{\qhF}{\hat\qF}
    \newcommand{\qbh}{\bar\qh}
    \newcommand{\qbn}{\bar\qn}

    \newcommand{\qwbE}{\overline{\bf E}}
    \newcommand{\qwbF}{\overline{\bf F}}
    \newcommand{\qwbT}{\overline{\bf T}}
    \newcommand{\qwbR}{\overline{\bf R}}

    \newcommand{\qDelta}{{\boldsymbol \Delta}}
    \newcommand{\qPsi}{{\boldsymbol \Psi}}
    \newcommand{\qPhi}{{\boldsymbol \Phi}}
    \newcommand{\qXi}{{\boldsymbol \Xi}}
    \newcommand{\qTheta}{{\boldsymbol \Theta}}
    \newcommand{\qLambda}{{\boldsymbol \Lambda}}
    \newcommand{\qSigma}{{\boldsymbol \Sigma}}
    \newcommand{\qGamma}{{\boldsymbol \Gamma}}
    \newcommand{\qUpsilon}{{\boldsymbol \Upsilon}}
    \newcommand{\qOmega}{{\boldsymbol \Omega}}
    \newcommand{\qPi}{{\boldsymbol \Pi}}

    \newcommand{\qalpha}{{\boldsymbol \alpha}}
    \newcommand{\qbeta}{{\boldsymbol \beta}}
    \newcommand{\qdelta}{{\boldsymbol \delta}}
    \newcommand{\qlambda}{{\boldsymbol \lambda}}
    \newcommand{\qgamma}{{\boldsymbol \gamma}}
    \newcommand{\qepsilon}{{\boldsymbol \epsilon}}
    \newcommand{\qeta}{{\boldsymbol \eta}}
    \newcommand{\qnu}{{\boldsymbol \nu}}
    \newcommand{\qmu}{{\boldsymbol \mu}}
    \newcommand{\qkappa}{{\boldsymbol \kappa}}
    \newcommand{\qtau}{{\boldsymbol \tau}}
    \newcommand{\qxi}{{\boldsymbol \xi}}
    \newcommand{\qzeta}{{\boldsymbol \zeta}}
    \newcommand{\qvarepsilon}{{\boldsymbol \varepsilon}}
    \newcommand{\qomega}{{\boldsymbol \omega}}

    \newcommand{\tH}{{\tilde{H}}}
    \newcommand{\tQ}{{\tilde{Q}}}
    \newcommand{\talpha}{{\tilde{\alpha}}}
    \newcommand{\ttau}{{\tilde{\tau}}}

    \newcommand{\tb}{{\tilde{b}}}
    \newcommand{\tc}{{\tilde{c}}}
    \newcommand{\te}{{\tilde{e}}}
    \newcommand{\tm}{{\tilde{m}}}
    \newcommand{\tq}{{\tilde{q}}}
    \newcommand{\tv}{{\tilde{v}}}
    \newcommand{\trho}{{\tilde{\rho}}}
    \newcommand{\tvarepsilon}{{\tilde{\varepsilon}}}

    \newcommand{\tqh}{{\tilde{\qh}}}
    \newcommand{\tqv}{{\tilde{\qv}}}
    \newcommand{\tqH}{{\tilde{\qH}}}
    \newcommand{\tqU}{{\tilde{\qU}}}
    \newcommand{\tqV}{{\tilde{\qV}}}
    \newcommand{\tqD}{{\tilde{\qD}}}
    \newcommand{\tqQ}{{\tilde{\qQ}}}
    \newcommand{\tchi}{{\tilde{\chi}}}
    \newcommand{\tqTheta}{{\tilde{\qTheta}}}
    \newcommand{\tqDelta}{{\tilde{\qDelta}}}
    \newcommand{\tqPsi}{{\tilde{\qPsi}}}
    \newcommand{\tqPhi}{{\tilde{\qPhi}}}
    \newcommand{\tcalqS}{{\tilde{\calqS}}}
    \newcommand{\tqXi}{{\tilde{\qXi}}}

    \newcommand{\tqLambda}{{\tilde{\qLambda}}}

    \newcommand{\hQ}{{\hat{Q}}}

    %\newcommand{\hm}{{\hat{m}}}
    \newcommand{\hchi}{{\hat{\chi}}}

    \newcommand{\hr}{{\hat{r}}}
    \newcommand{\hs}{{\hat{s}}}
    \newcommand{\hq}{{\hat{q}}}
    \newcommand{\hp}{{\hat{p}}}
    \newcommand{\bp}{{\bar{p}}}
    \newcommand{\bv}{{\bar{v}}}
    \newcommand{\bH}{{\bar{H}}}
    \newcommand{\bqH}{{\bar{\qH}}}

    \newcommand{\whqX}{{\widehat{\qX}}}
    \newcommand{\whqZ}{{\widehat{\qZ}}}
    \newcommand{\whqH}{{\widehat{\qH}}}
    \newcommand{\whX}{{\widehat{X}}}
    \newcommand{\whH}{{\widehat{H}}}
    \newcommand{\whZ}{{\widehat{Z}}}

    \newcommand{\wtqY}{{\widetilde{\qY}}}
    \newcommand{\wtY}{{\widetilde{Y}}}
    \newcommand{\wty}{{\widetilde{y}}}


    \newcommand{\uqB}{{\underline{\qB}}}
    \newcommand{\uH}{{\underline{H}}}
    \newcommand{\utH}{{\underline{\tH}}}
    \newcommand{\ubH}{{\underline{\bH}}}
    \newcommand{\uR}{{\underline{R}}}
    \newcommand{\uT}{{\underline{T}}}
    \newcommand{\uqH}{{\underline{\qH}}}
    \newcommand{\uqR}{{\underline{\qR}}}
    \newcommand{\uqT}{{\underline{\qT}}}
    \newcommand{\ubqH}{{\underline{\bqH}}}
    \newcommand{\utqH}{{\underline{\tqH}}}
    \newcommand{\ucalqX}{{\underline{\calqX}}}
    \newcommand{\uqX}{{\underline{\qX}}}

    \newcommand{\bbB}{{\mathbb B}}
    \newcommand{\bbE}{{\mathbb E}}
    \newcommand{\bbN}{{\mathbb N}}
    \newcommand{\bbR}{{\mathbb R}}
    \newcommand{\bbC}{{\mathbb C}}
    \newcommand{\bbS}{{\mathbb S}}
    \newcommand{\bbU}{{\mathbb U}}
    \newcommand{\bbQ}{{\mathbb Q}}

    \newcommand{\calA}{{\mathcal A}}
    \newcommand{\calB}{{\mathcal B}}
    \newcommand{\calC}{{\mathcal C}}
    \newcommand{\calD}{{\mathcal D}}
    \newcommand{\calE}{{\mathcal E}}
    \newcommand{\calF}{{\mathcal F}}
    \newcommand{\calG}{{\mathcal G}}
    \newcommand{\calI}{{\mathcal I}}
    \newcommand{\calK}{{\mathcal K}}
    \newcommand{\calL}{{\mathcal L}}
    \newcommand{\calM}{{\mathcal M}}
    \newcommand{\calN}{{\mathcal N}}
    \newcommand{\calS}{{\mathcal S}}
    \newcommand{\calT}{{\mathcal T}}
    \newcommand{\calO}{{\mathcal O}}
    \newcommand{\calQ}{{\mathcal Q}}
    \newcommand{\calR}{{\mathcal R}}
    \newcommand{\calV}{{\mathcal V}}
    \newcommand{\calX}{{\mathcal X}}

    \newcommand{\calqA}{\boldsymbol{\cal A}}
    \newcommand{\calqB}{\boldsymbol{\cal B}}
    \newcommand{\calqH}{\boldsymbol{\cal H}}
    \newcommand{\calqX}{\boldsymbol{\cal X}}
    \newcommand{\calqQ}{\boldsymbol{\cal Q}}
    \newcommand{\calqS}{\boldsymbol{\cal S}}
    \newcommand{\calqZ}{\boldsymbol{\cal Z}}



    \newcommand{\dom}{{\sf dom}}
    \newcommand{\epi}{{\sf epi}}
    \newcommand{\diag}{{\sf diag}}
    \newcommand{\supp}{{\sf supp}}
    \newcommand{\tr}{{\sf tr}}
    \newcommand{\Ex}{{\sf E}}
    \newcommand{\rank}{{\sf rank}}
    \newcommand{\Varx}{{\sf Var}}
    \newcommand{\Extr}{\operatornamewithlimits{\sf Extr}}
    \newcommand{\mmse}{{\sf mmse}}
    \newcommand{\mse}{{\sf mse}}
    \newcommand{\vect}{{\sf vec}}
    \newcommand*{\argmin}{\operatornamewithlimits{argmin}\limits}
    \newcommand*{\argmax}{\operatornamewithlimits{argmax}\limits}
    \newcommand{\sfQ}{{\sf Q}}
    \newcommand{\sign}{{\sf sign}}


    \newcommand{\rmd}{{\rm d}}
    \newcommand{\rmD}{{\rm D}} 

    \newcommand{\sfa}{{\sf a}}
    \newcommand{\sfb}{{\sf b}}
    \newcommand{\sfc}{{\sf c}}
    \newcommand{\sfd}{{\sf d}}
    \newcommand{\sfe}{{\sf e}}
    \newcommand{\sff}{{\sf f}}
    \newcommand{\sfg}{{\sf g}}
    \newcommand{\sfh}{{\sf h}}
    \newcommand{\sfi}{{\sf i}}
    \newcommand{\sfj}{{\sf j}}
    \newcommand{\sfk}{{\sf k}}
    \newcommand{\sfl}{{\sf l}}
    \newcommand{\sfm}{{\sf m}}
    \newcommand{\sfn}{{\sf n}}
    \newcommand{\sfo}{{\sf o}}
    \newcommand{\sfp}{{\sf p}}
    \newcommand{\sfq}{{\sf q}}
    \newcommand{\sfr}{{\sf r}}
    \newcommand{\sfs}{{\sf s}}
    \newcommand{\sft}{{\sf t}}
    \newcommand{\sfu}{{\sf u}}
    \newcommand{\sfv}{{\sf v}}
    \newcommand{\sfw}{{\sf w}}
    \newcommand{\sfx}{{\sf x}}
    \newcommand{\sfy}{{\sf y}}
    \newcommand{\sfz}{{\sf z}}




    \newcommand{\sfB}{{\sf B}}
    \newcommand{\sfC}{{\sf C}}
    \newcommand{\sfF}{{\sf F}}
    \newcommand{\sfH}{{\sf H}}
    \newcommand{\sfP}{{\sf P}}
    \newcommand{\sfX}{{\sf X}}
    \newcommand{\sfZ}{{\sf Z}}
    \newcommand{\sfqB}{\boldsymbol{\sf B}}
    \newcommand{\sfqH}{\boldsymbol{\sf H}}
    \newcommand{\sfqX}{\boldsymbol{\sf X}}
    \newcommand{\sfqx}{\boldsymbol{\sf x}}
    \newcommand{\sfqh}{\boldsymbol{\sf h}}

    \newcommand{\scP}{\mathscr{P}}
    \newcommand{\scF}{\mathscr{F}}

    \newcommand{\aaa}{\buildrel{\circ}\over{a}}
    \newcommand{\aag}{\buildrel{\circ}\over{g}}
    \newcommand{\aeta}{\buildrel{\circ}\over{\eta}}
    \newcommand{\arho}{\buildrel{\circ}\over{\rho}}
    \newcommand{\aalpha}{\buildrel{\circ}\over{\alpha}}
    \newcommand{\ateta}{\buildrel{\circ}\over{\tilde\eta}}
    \newcommand{\atalpha}{\buildrel{\circ}\over{\tilde\alpha}}
    \newcommand{\atrho}{\buildrel{\circ}\over{\tilde\rho}}


    \newcommand{\bfbl}[1]{\bf \color{blue}#1}
    \newcommand{\bl}[1]{\color{blue}#1}
    \newcommand{\bfrl}[1]{\bf \color{red}#1}
    \newcommand{\rl}[1]{\color{red}#1}
    \newcommand{\bfbrl}[1]{\bf \color{BrickRed}#1}
    \newcommand{\bfbbl}[1]{\bf \color{BlueViolet}#1}




    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

